Class-based Subset Selection for Transfer Learning under Extreme Label Shift

Existing work within transfer learning often follows a two-step process -- pre-training over a large-scale source domain and then finetuning over limited samples from the target domain. Yet, despite its popularity, this methodology has been shown to suffer in the presence of distributional shift -- specifically when the output spaces diverge. Previous work has focused on increasing model performance within this setting by identifying and classifying only the shared output classes between distributions. However, these methods are inherently limited as they ignore classes outside the shared class set, disregarding potential information relevant to the model transfer. This paper proposes a new process for few-shot transfer learning that selects and weighs classes from the source domain to optimize the transfer between domains. More concretely, we use Wasserstein distance to choose a set of source classes and their weights that minimize the distance between the source and target domain. To justify our proposed algorithm, we provide a generalization analysis of the performance of the learned classifier over the target domain and show that our method corresponds to a bound minimization algorithm. We empirically demonstrate the effectiveness of our approach (WaSS) by experimenting on several different datasets and presenting superior performance within various label shift settings, including the extreme case where the label spaces are disjoint.

==> figures/figure3.tex <==
\begin{figure*}[h!]
\centering
	\begin{subfigure}[]{0.49\textwidth}
		\includegraphics[width=\textwidth]{figures/fmnist_after.png}
		\caption{Fashion-MNIST}
		\label{fig:vis_after:mnist}
	\end{subfigure}
	\begin{subfigure}[]{0.49\textwidth}
		\includegraphics[width=\textwidth]{figures/cifar10_after.png}
		\caption{CIFAR 10}
		\label{fig:vis_after:cifar10}
	\end{subfigure}
	%\begin{subfigure}[]{0.32\textwidth}
	%	\includegraphics[width=\textwidth]{figures/pacs_after.png}
	%	\caption{PACS}
	%	\label{fig:vis_after:pacs}
	%\end{subfigure}
    \caption{}
    \label{fig:vis_after}
\end{figure*}

==> genrealizationBound-Temp.tex <==

\section{Proof of \ref{lemma:transfer}}

\textbf{Lemma \ref{lemma:transfer} (Error bound on pre-trained and fine-tuned model)} 

Given two classifiers $h,h'$ that only differ by their final layer, we can bound their error as following:
\begin{align*}
   \epsilon_T(h') \leq \epsilon_S(h) + \alpha \beta \sigma_{\max} (V_{S}-V_{T})
\end{align*}


\emph{Proof:}

Define S and T somewhere. Also define error $\epsilon$

\subsection{Theorem 1: Proof of Bound with disjoint source and target label spaces}
$$ \epsilon_T(h) \leq \epsilon_s(h) + \rho W_1 $$

\subsection{Lemma 1: }
Proof of: \\
Define the softmax function $\sigma : x_i \mapsto \exp(x_i) / \sum_j exp(x_j)$ with Lipschitz constant $\alpha = \frac{\sqrt{K-1}}{K}$  $\forall K \geq 2 \cite{gao1704properties}$.
$ \forall v, v' $,
$$ ||\sigma(v) - \sigma(v') ||_1 \leq  \alpha ||v-v'||_2$$

\subsection{Lemma 2: The $L_2$ norm of a vector is bounded by its largest singular value. }

\subsection{Theorem 2: Proof of Bound with finetuning of linear classification head}
Consider a pretrained classifier $h^o$ and a finetuned classifier $h^*$ which only differ in the final classification layer. Given an input space $X \subset \mathbb{R}^d$, the classifiers first consist of a feature map $W : X \to F$. Assume the features are bounded $||W(x)||_2 \leq \beta$ $\forall x \in X$. For each classifier, these features are mapped to logits using matrices $O, Z \in \mathbb{R}^{k \times d}$ for the pretrained and finetuned classifiers, respectively: $h^o : x \mapsto OW(x)$ and $h^* : x \mapsto ZW(x)$. By Theorem 1,

$$ \epsilon_T(h^o) \leq \epsilon_S(h^o) + \rho W_1 $$
$$ \epsilon_T(h^o) \leq \epsilon_S(h^o) + \rho W_1 + (\epsilon_S(h^*) - \epsilon_S(h^*))$$
$$ \epsilon_T(h^o) \leq \epsilon_S(h^*) + \rho W_1 + (\epsilon_S(h^o) -\epsilon_S(h^*)) $$
Now, we will consider the final term $\epsilon_S(h^o) -\epsilon_S(h^*)$ on the right hand side. With labeling function $Y : X \to \mathbb{R}^k$, 
$$\epsilon_S(h^o) -\epsilon_S(h^*) = \E X_S ||Y(x) - \sigma(OW(x))||_1 - \E X_S||Y(x) - \sigma(ZW(x))||_1$$
$$= \E_{X_S} \left[ ||Y(x) - \sigma(OW(x))||_1 - ||Y(x) - \sigma(ZW(x))||_1 \right]$$
By triangle inequality, 
%$$\EX_S \left[ ||f(x) - \sigma(OW(x))|| - ||f(x) - \sigma(ZW(x))||_1 \right] $$
$$\leq \E_{X_S} \left[ ||Y(x) - \sigma(OW(x)) - Y(x) + \sigma(ZW(x))||_1 \right] $$
$$= \E X_S ||\sigma(ZW(x)) - \sigma(OW(x))||_1 $$
By Lemma 1,
$$ \E_{X_S} \left[ ||\sigma(ZW(x)) - \sigma(OW(x))||_1 \right] \leq \alpha ||ZW(x)-OW(x)||_2 $$
$$ = \alpha ||(Z-O)W(x)||_2 \leq \alpha ||Z-O||_2 \beta$$
given we assume that all our features are bounded. Finally, using Lemma 2, we can bound $Z-O$ by its largest singular value $\sigma_{\max}$,
$$\alpha \beta ||(Z-O)||_2 \leq \alpha \beta \sigma_{\max} (Z-O)$$
Putting it all together, we get
$$\epsilon_T(h^o) \leq \epsilon_S(h^*) + \rho W_1 + \alpha \beta \sigma_{\max} (Z-O)$$
$\square$

If we assume no finetuning is done ($h^o = h^* \iff Z = O$), we see that this collapses to Theorem 1. 


\newpage

% \textbf{Proof} Let $\mu, \nu$ represent the joint distributions $D_S, D_T$ respectively, $P(\mu, \nu)$ be the set of joint distribution between $\mu, \nu$.
% \begin{align}
%         W_1(\gD_S, \gD_T) &= \inf _{\gamma \in P(\mu, \nu)} \mathop{\mathbb{E}}_{(Z,Y; Z',Y')\sim \gamma}[c(Z,Y; Z',Y')]\\
%         &= \inf _{\gamma \in P(\mu, \nu)} \mathop{\mathbb{E}}_{(Z,Y; Z',Y')\sim \gamma}[c_1(Z, Z')] + \inf _{\gamma \in P(\mu, \nu)} \mathop{\mathbb{E}}_{(Z,Y; Z',Y')\sim \gamma}[c_2(Y,Y')]\\
%         &= \inf _{\gamma \in P(Z, Z')} \mathop{\mathbb{E}}_{(Z, Z')\sim \gamma}[c_1(Z, Z')] + \inf _{\gamma \in P(Y, Y')} \mathop{\mathbb{E}}_{(Y, Y')\sim \gamma}[c_2(Y,Y')]\\
%         &= W_1(\gD_S(Z), \gD_T(Z)) + \inf _{\gamma \in P(\mu, \nu)} \mathop{\mathbb{E}}_{(Y, Y')\sim \gamma}[c_2(Y,Y')]
%     \end{align}
%     Line $6$ holds because the variable pair $(Z, Z')$ is independent of $(Y, Y')$. Line $7$ holds because  $P(Z, Z')$ and $P(Y, Y')$ are marginals on $(Z, Z')$ and $(Y, Y')$ respectively induced on the joint distribution $P(\mu, \nu)$. Line $8$ is the definition of Wasserstein distance over the marginal distribution on the $X$ axis.

==> tables/table2.tex <==
\begin{table}[htp]
  \caption{Open set class setting on MNIST-Fashion \carl{In original paper I think this is Fashion-MNIST?} (M-Fash), Cifar 10 (C-10), PACS (P), Cifar 100 (C-100). The accuracy of the downstream classifier and T.V. distance of class weights chosen by each method are shown. Test classes for each dataset are fixed at $[0,1,2]$ \carl{Can we give an example of training classes then? e.g. CIFAR-10 is $[3, 4, 5, 6, 7, 8, 9, 0, 1]$}}
  \label{tab:results_table2}
  \centering
  \setlength{\tabcolsep}{0pt} 
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}\quad}llll}
\hline
Dataset &             & OSS   & WaSS   \\ \hline
\multirow{2}{*}{M-Fash} & Accuracy    & 95.86 & \textbf{95.98}  \\ 
                        & TV Distance & 0.010 & 0.013  \\ 
\multirow{2}{*}{C-10}   & Accuracy    & 81.80 & \textbf{90.66}  \\ 
                        & TV Distance & 0.18  & 0.077  \\
\multirow{2}{*}{PACS}   & Accuracy    & 51.40 & \textbf{73.39}  \\ 
                        & TV Distance & 0.009 & 0.0123 \\ 
\multirow{2}{*}{C-100}  & Accuracy    & 45.63 & \textbf{62.00}  \\ 
                        & TV Distance & 0.003 & 0.016 \\ \hline
\end{tabular*}
\end{table}

==> tables/table3.tex <==
\begin{table}[htb]
  \caption{Accuracy of varied layer downstream classifier given a varied length feature vector on MNIST-Fashion (M-Fash), Cifar 10 (C-10), PACS (P), Cifar 100 (C-100). Best performing results are bolded. Test classes for each dataset are fixed at $[0,1,2]$}
  \label{tab:open-set}
  \centering
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}\quad}llll}
\hline
Dataset                      & Feature Length              & ALL                        & WaSS                                \\ \hline
\multirow{2}{*}{M-Fash} & \multicolumn{1}{l}{64}   & \multicolumn{1}{l}{74.12} & \multicolumn{1}{l}{\textbf{79.76}} \\ 
     & \multicolumn{1}{l}{256}  & \multicolumn{1}{l}{63.79} & \multicolumn{1}{l}{\textbf{79.43}} \\ 
\multirow{2}{*}{C-10}   & \multicolumn{1}{l}{64}   & \multicolumn{1}{l}{76.19} & \multicolumn{1}{l}{\textbf{77.08}} \\ 
     & \multicolumn{1}{l}{256}  & \multicolumn{1}{l}{79.03} & \multicolumn{1}{l}{\textbf{80.03}} \\ 
\multirow{2}{*}{PACS}   & \multicolumn{1}{l}{64}  & \multicolumn{1}{l}{44.11} & \multicolumn{1}{l}{\textbf{61.24}} \\ 
   & \multicolumn{1}{l}{256}  & \multicolumn{1}{l}{50.12} & \multicolumn{1}{l}{\textbf{68.25}} \\ 
\multirow{2}{*}{C-100}  & \multicolumn{1}{l}{64}   & \multicolumn{1}{l}{49.24} & \multicolumn{1}{l}{\textbf{56.9}}  \\ 
      & \multicolumn{1}{l}{256}  & \multicolumn{1}{l}{50.67} & \multicolumn{1}{l}{\textbf{80.03}} \\ \hline
\end{tabular*}
\end{table}
